Practical Issues of Energy Harvesting and Data Transmissions in Sustainable IoT

The sustainable Internet of Things (IoT) is becoming a promising solution for the green living and smart industries. In this article, we investigate the practical issues in the radio energy harvesting and data communication systems through extensive field experiments. A number of important characteristics of energy harvesting circuits and communication modules have been studied, including the non-linear energy consumption of the communication system relative to the transmission power, the wake-up time associated with the payload, and the varying system power during consecutive packet transmissions. In order to improve the efficiency of energy harvest and energy utilization, we propose a new model to accurately describe the energy harvesting process and the power consumption for sustainable IoT devices. Experiments are performed using commercial IoT devices and RF energy harvesters to verify the accuracy of the proposed model. The experiment results show that the new model matches the performance of sustainable IoT devices very well in the real scenario.

==> TranStrategy.tex <==
\section{Optimal Transmission Strategy}
\label{sec:TranStrategy}

In this section, we study the optimal transmission strategy based on our energy consumption model to maximize the throughput of RF-powered sustainable IoT devices. 



























